Universal Properties of Lens Proxy Pullbacks

A comprehensive account of the categorical properties of the category of small categories and asymmetric delta lenses is given in the recent works of Chollet et al. and Di Meglio. An important construction for proving many of these properties is Johnson and Rosebrugh's "pullback" of lenses, which we call the proxy pullback of lenses. We give a new treatment of the proxy pullback in terms of compatibility, a stronger notion of commutativity for squares of lenses. The proxy pullback is sometimes, but not always, a real pullback. Using new notions of sync-minimal and independent lens spans, we characterise when a lens span that forms a commuting square with a lens cospan has a comparison lens to a proxy pullback of the cospan.

==> eptcsdata.tex <==
\providecommand{\firstpage}{400}
\providecommand{\publicationstatus}{J. Master \& M. Lewis (Eds.): Fifth International\\
Conference on Applied Category Theory (ACT 2022).\\
EPTCS 380, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.380.23}{10.4204/EPTCS.380.23}}
\pdfoutput=1


==> preamble/colors.tex <==
\definecolor{MQRed}{RGB}{166,25,46}
\definecolor{MQDeepRed}{RGB}{118,35,47}
\definecolor{MQBrightRed}{RGB}{214,0,28}
\definecolor{MQMagenta}{RGB}{198,0,126}
\definecolor{MQPurple}{RGB}{128,34,95}
\definecolor{MQCharcoal}{RGB}{55,58,54}
\definecolor{MQSand}{RGB}{214,210,196}
\definecolor{MyGrey}{RGB}{229,229,232}

==> preamble/commands.tex <==
% REMEMBER:
% \mathrel for binary relations, eg. =
% \mathbin for binary operators, eg. +,-
% \mathop for unary operators, eg. \sum, \cos, \sin
% \mathord
% \mathopen
% \mathclose
% \mathpunct

% OVERLINE
\newcommand{\overCap}[1]{\mskip.5\thinmuskip\overline{\mskip-.5\thinmuskip {#1} \mskip-.5\thinmuskip}\mskip.5\thinmuskip}
\newcommand{\overCapIt}[1]{\,\overline{\!{#1}}}


% LARGE CATEGORIES
\newcommand{\unkernBig}{\mkern-1.8mu}
\newcommand{\unkernSmall}{\mkern-1mu}


\newcommand{\largeCat}[2]{\mathit{\mathscr{#1} \unkernBig {#2}}}
% \newcommand{\largeCat}[1]{\mathord{\mathsf{#1}}}
% \newcommand{\largeCat}[1]{\mathrm{\mathscr#1}}
\newcommand{\Cat}{\largeCat{C}{at}}
\newcommand{\Top}{\largeCat{T}{op}}
\newcommand{\Set}{\largeCat{S}{et}}
\newcommand{\Cof}{\largeCat{C}{of}}
\newcommand{\Lens}{\largeCat{L}{ens}}  %{\largeCat{Lens}}
\newcommand{\Span}{\largeCat{S}{pan}}
\newcommand{\CofSq}{\mathit{\mathscr{C} \unkernBig of \unkernSmall \mathscr{S} \unkernBig q}}
\newcommand{\SymLens}{\mathit{\mathscr{S} \unkernBig ym \unkernSmall \mathscr{L} \unkernBig ens}}
\newcommand{\SpanLens}{\mathit{\mathscr{S} \unkernBig pan \unkernSmall \mathscr{L} \unkernBig ens}}

\newcommand{\forget}{\mathscr{G}}
\newcommand{\forgetLensToCat}{\forget}
\newcommand{\forgetLensToSet}{\mathscr{W}}
\newcommand{\forgetLensToCof}{\mathscr{P}}
\newcommand{\forgetCatToSet}{\mathscr{U}}
\newcommand{\forgetCofToSet}{\mathscr{V}}

\newcommand{\Src}{\mathscr{S}}
\newcommand{\Tgt}{\mathscr{T}}

\newcommand{\Filter}{\mathscr{F}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\M}{\mathcal{M}}


\newcommand{\V}{\mathcal{V}}

\newcommand{\PPB}{\mathsf{PPB}}

\newcommand{\Adiagram}{\mathscr{A}}
\newcommand{\Bdiagram}{\mathscr{B}}
\newcommand{\Fdiagram}{\mathscr{F}}


% DOUBLE CATEGORIES
\newcommand{\doubleCat}[2]{\mathit{\mathbb{#1}\unkernSmall{#2}}}
\newcommand{\RRel}{\doubleCat{R}{el}}
\newcommand{\SSpan}{\mathop{\doubleCat{S}{pan}}}
\newcommand{\MMat}{\mathop{\doubleCat{M}{at}}}
\newcommand{\CComod}{\mathop{\doubleCat{C}{omod}}}
\newcommand{\FFil}{\doubleCat{F}{ltr}}
\newcommand{\TTop}{\doubleCat{T}{op}}
\newcommand{\MMnd}{\mathop{\doubleCat{M}{nd}}}
\newcommand{\CCof}{\mathop{\doubleCat{C}{of}}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\CC}{\mathbb{C}}


% SMALL CATEGORIES
\newcommand{\smallCat}{\mathbf}
\newcommand{\terminalCat}{\smallCat{1}}
\newcommand{\intervalCat}{\smallCat{2}}
\newcommand{\isomorphismCat}{\smallCat{I}}
\newcommand{\A}{\smallCat{A}}
\newcommand{\J}{\smallCat{J}}
\newcommand{\Abar}{\overCap{\A}}
\newcommand{\B}{\smallCat{B}}
\newcommand{\Bbar}{\overCap{\B}}
\newcommand{\D}{\smallCat{D}}
\newcommand{\E}{\smallCat{E}}
\newcommand{\C}{\smallCat{C}}
\newcommand{\K}{\smallCat{K}}
\DeclareMathOperator{\Ker}{\smallCat{Ker}}
\DeclareMathOperator{\Coker}{\smallCat{Coker}}
\DeclareMathOperator{\Eq}{\smallCat{Eq}}
\DeclareMathOperator{\Coeq}{\smallCat{Coeq}}
\DeclareMathOperator{\Image}{\smallCat{Im}}

% FUNCTORS
\newcommand{\Ebar}{\overCapIt{E}}
\newcommand{\Fbar}{\overCapIt{F}}
\newcommand{\Gbar}{\overCapIt{G}}
\newcommand{\Hbar}{\overCapIt{H}}
\newcommand{\Jbar}{\overCapIt{J}}
\newcommand{\Kbar}{\overCapIt{K}}
\newcommand{\Lbar}{\overCapIt{L}}


% OBJECTS
\newcommand{\Ybar}{\overCapIt{Y}}
\newcommand{\Xbar}{\overCapIt{X}}
\newcommand{\Zbar}{\overCapIt{Z}}
\newcommand{\Wbar}{\overCapIt{W}}
\newcommand{\fbar}{\overCapIt{f}}


% SETS
\DeclarePairedDelimiterX{\setb}[2]{\lbrace}{\rbrace}{#1:\;#2}
\DeclarePairedDelimiter{\set}{\lbrace}{\rbrace}
\newcommand{\setDifference}{\mathbin{\backslash}}
\newcommand{\DisjointUnion}{\bigsqcup}

% CLASSES
\newcommand{\class}{\mathcal}
\newcommand{\monoClass}{\class{M}}
\newcommand{\epiClass}{\class{E}}
\newcommand{\leftOrthogonalClass}[1]{{{}^{\perp}}{#1}}
\newcommand{\rightOrthogonalClass}[1]{{#1}^{\perp}}

% % CATEGORY THEORY
\DeclarePairedDelimiter{\objectSet}{\lvert}{\rvert}
\DeclarePairedDelimiterXPP{\homSet}[3]{#1}{(}{)}{}{#2, #3}
\DeclarePairedDelimiterXPP{\outSet}[2]{#1}{(}{)}{}{#2, \ast}

\DeclareMathOperator{\source}{src}
\DeclareMathOperator{\target}{tgt}

\newcommand{\id}[1]{\operatorname{id}_{#1}}
\newcommand{\compose}{\mathbin{\circ}}
\newcommand{\sequence}{\mathbin{\fatsemi}}

\newcommand*{\coColon}{%
    \nobreak
    \mskip6mu plus1mu
    \mathpunct{}%
    \nonscript
    \mkern-\thinmuskip
    {:}%
    \mskip2mu
    \relax
}

\newcommand{\coTo}{\leftarrow}
\newcommand{\monicTo}{\rightarrowtail}
\newcommand{\epicTo}{\twoheadrightarrowtail}
\DeclarePairedDelimiterX{\pair}[2]{\langle}{\rangle}{#1, \, #2}
\DeclarePairedDelimiterX{\copair}[2]{[}{]}{#1, \, #2}
\newcommand{\pullback}[1]{\mathbin{\times_{#1}}}
\newcommand{\pushout}[1]{\mathbin{\sqcup_{#1}}}
% \newcommand{\identifyRel}[2]{\mathrel{{{}_{#1}}{\equiv}_{#2}}}

% LENSES
\newcommand{\lift}[2]{{#1}{}^{#2}}
\newcommand{\PutId}{PutId}
\newcommand{\PutPut}{PutPut}
\newcommand{\PutGet}{PutGet}
\newcommand{\PutTgt}{PutTgt}
\newcommand{\GetPut}{GetPut}
\newcommand{\onlyIfDirection}{\textit{only if} direction}
\newcommand{\ifDirection}{\textit{if} direction}

\newcommand{\freeProduct}{\mathbin{\Box}}

% BRACKETS
\DeclarePairedDelimiter{\paren}{(}{)}
\let\brack\undefined
\DeclarePairedDelimiter{\brack}{[}{]}
\let\angle\undefined
\DeclarePairedDelimiter{\angle}{\langle}{\rangle}

% PHRASES

\newcommand{\sync}{\mathscr{M}}
\newcommand{\syncCounit}[1]{E_{#1}}


% =============================================
%Import symbols from font cm without importing the whole package
% =============================================
\newcommand\imCMsym[4][\mathord]{%
  \DeclareFontFamily{U} {#2}{}
  \DeclareFontShape{U}{#2}{m}{n}{
    <-6> #25
    <6-7> #26
    <7-8> #27
    <8-9> #28
    <9-10> #29
    <10-12> #210
    <12-> #212}{}
  \DeclareSymbolFont{CM#2} {U} {#2}{m}{n}
  \DeclareMathSymbol{#4}{#1}{CM#2}{#3}
}
\newcommand\alsoimCMsym[4][\mathord]{\DeclareMathSymbol{#4}{#1}{CM#2}{#3}}

% \imCMsym{cmmi}{124}{\CMjmath}
% \imCMsym[\mathop]{cmsy}{113}{\CMamalg}
\imCMsym[\mathop]{cmex}{96}{\smallcoprod}
\alsoimCMsym[\mathop]{cmex}{97}{\Coprod}

==> preamble/environments.tex <==
% \numberwithin{section}{chapter}

\newtheorem{theorem}                    {Theorem} [section]
\newtheorem{lemma}          [theorem]   {Lemma}
\newtheorem{proposition}    [theorem]   {Proposition}
\newtheorem{corollary}      [theorem]   {Corollary}
\newtheorem{conjecture}     [theorem]   {Conjecture}

\theoremstyle{definition}
\newtheorem{definition}     [theorem]   {Definition}
\newtheorem{example}        [theorem]   {Example}

\theoremstyle{remark}
\newtheorem{remark}         [theorem]   {Remark}
\newtheorem{warning}         [theorem]   {Warning}

% \usepackage{chngcntr}
% \counterwithout*{equation}{section}
% \numberwithin{equation}{chapter}
% \renewcommand{\theequation}{\arabic{equation}}

==> preamble/other.tex <==
\crefname{equation}{}{}
\Crefname{equation}{}{}
\crefname{enumi}{}{}
\Crefname{enumi}{}{}

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}

% \numberwithin{equation}{section}

==> preamble/packages.tex <==
% OTHER PACKAGES
\usepackage[utf8]{inputenc}
\usepackage[mathscr]{eucal} % For curly categories
\usepackage[colorinlistoftodos]{todonotes} % disable
\usepackage{stmaryrd} % for fat semi
\usepackage{lipsum}
\usepackage{microtype} % for nicer typography
% \usepackage[svgnames]{xcolor}
\usepackage{xparse}

\usepackage{csquotes}
\usepackage[vskip=0pt,begintext=\textooquote,endtext=\textcoquote]{quoting}

\usepackage{tabularx}
\usepackage{calc} % For computations in setlengtgh

% AMS PACKAGES
\usepackage{amsmath}
\usepackage{amsthm} % For theorem environments
\usepackage{amssymb}
\usepackage{mathtools} % For paired delimiters

% DIAGRAM PACKAGES
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage[shortlabels]{enumitem}

% REFERENCING
\input{preamble/colors}
\usepackage[capitalize, noabbrev, nameinlink]{cleveref}
\usepackage[square,numbers]{natbib}

% FONTS
\usepackage{mathrsfs}
\let\curlyscr\mathscr
\usepackage[mathscr]{eucal} % For category and functor names

==> preamble/tikz.tex <==
\usetikzlibrary{decorations.markings}
\usetikzlibrary{fit}

\newcommand{\arrowLength}{2.3pt}
\newcommand{\arrowWidth}{4.6pt}

\tikzcdset{
    mark/.style={
        postaction={
            decorate,
            decoration={
                markings,
                mark={#1}
            },
        },
    },
    wideMark/.style={
        labels={
            inner sep=0.8ex,
        },
    },
    morphismTip/.tip={Triangle[length=\arrowLength, width=\arrowWidth]},
    lensTip/.tip={Diamond[length=2*\arrowLength, width=\arrowWidth]},
    functor/.style={
        wideMark,
        mark=at position {0.5*\pgfdecoratedpathlength + \arrowLength} with {\arrow{morphismTip}},
    },
    cofunctor/.style={
        wideMark,
        mark=at position {0.5*\pgfdecoratedpathlength - \arrowLength} with {\arrowreversed{morphismTip}},
    },
    lens/.style={
        wideMark,
        mark=at position {0.5*\pgfdecoratedpathlength + \arrowLength} with {\arrow{lensTip}},
    },
    proarrow/.style={
        wideMark,
        mark=at position 0.5 with {\draw[-] (0,-2.5pt) -- (0,2.5pt);}
    },
    cell/.style={
        phantom,
        "\xRightarrow{#1}",
    },
    cellUnlabelled/.style={
        phantom,
        "\Rightarrow",
    },
    PPB/.style={
        phantom, "\PPB"{font=\scriptsize}
    },
}

\tikzcdset{
    ar/.style={
        ampersand replacement=\&
    },
    upLeftAdjointTo/.style={
        phantom, "\vdash"{sloped, rotate=90, font=\scriptsize}
    }
}
\tikzset{
    boxed/.style={
        draw,
        thick,
        fill=black!5!white,
        rounded corners,
        % inner xsep=1ex,
        % inner ysep=0.85ex,
        outer xsep=1ex,
        outer ysep=0.85ex,
        inner sep=0pt,
        prefix after command={
            \pgfextra{\tikzset{
                every label/.style={
                    inner sep=0ex
                }
            }}
        }
    },
    description/.append style={
        inner ysep=0.5ex,
        inner xsep=0.1ex,
    },
}

